Topological Crystalline Bose Insulator in Two Dimensions via Entanglement Spectrum

Strongly correlated analogues of topological insulators have been explored in systems with purely on-site symmetries, such as time-reversal or charge conservation. Here, we use recently developed tensor network tools to study a quantum state of interacting bosons which is featureless in the bulk, but distinguished from an atomic insulator in that it exhibits entanglement which is protected by its spatial symmetries. These properties are encoded in a model many-body wavefunction that describes a fully symmetric insulator of bosons on the honeycomb lattice at half filling per site. While the resulting integer unit cell filling allows the state to bypass `no-go' theorems that trigger fractionalization at fractional filling, it nevertheless has nontrivial entanglement, protected by symmetry. We demonstrate this by computing the boundary entanglement spectra, finding a gapless entanglement edge described by a conformal field theory as well as degeneracies protected by the non-trivial action of combined charge-conservation and spatial symmetries on the edge. Here, the tight-binding representation of the space group symmetries plays a particular role in allowing certain entanglement cuts that are not allowed on other lattices of the same symmetry, suggesting that the lattice representation can serve as an additional symmetry ingredient in protecting an interacting topological phase. Our results extend to a related insulating state of electrons, with short-ranged entanglement and no band insulator analogue.

==> commands/pgfstyles.tex <==
\tikzset{peps/.style={circle=2pt,draw=black!100,fill=green!50,inner sep=3pt}}
\tikzset{bpeps/.style={circle=2pt,draw=black!100,thick,fill=green!50,inner sep=3pt}}
\tikzset{gamma/.style={circle=2pt,draw=black!100,fill=blue!20,inner sep=3pt}}
\tikzset{lambda/.style={rectangle,rotate=45,draw=black!100,fill=orange!50,inner sep=4pt}}
\tikzset{operator/.style={circle=2pt,draw=black!100,fill=orange!80,inner sep=3pt}}
\tikzset{cdot/.style={circle=2pt,draw=black!100,fill=white,inner sep=1pt}}
\tikzset{bg/.style={rounded corners,thin,fill=blue!10}}
\tikzset{inv/.style={opacity=0}}
\tikzset{spin/.style={circle=2pt,draw=black!100,fill=orange!80,inner sep=3pt}}
\tikzset{unitbox/.style={fill=black!3,rounded corners}}
\tikzset{corner/.style={rectangle=10pt,fill=blue!50,draw=black}}
\tikzset{side/.style={rectangle=6pt,fill=blue!20,draw=black}}
\tikzset{cside/.style={circle=6pt,fill=blue!20,draw=black}}
\tikzset{swapg/.style={circle=1pt,draw=black,fill=black!80,inner sep=1pt}}

\tikzset{base/.style={circle=2pt,fill=orange!80,draw=black}}
\tikzset{det/.style={circle=2pt,fill=blue!20,draw=black,inner sep=4pt}}
\tikzset{iso/.style={circle=2pt,fill=red!20,draw=black,inner sep=4pt}}
\tikzset{top/.style={circle=2pt,fill=black!20,draw=black,inner sep=4pt}}
\tikzset{siso/.style={circle=1pt,fill=red!20,draw=black,inner sep=1pt}}

%Brayden's
\tikzset{GHZ/.style={circle=2pt,fill=black!80,draw=black,inner sep=2pt}}
\tikzset{X/.style={circle=2pt,fill=black!80,text=white,font=\footnotesize, draw=black,inner sep=1pt}}
\tikzset{W/.style={circle=2pt,fill=black!20,draw=black,double,inner sep=2pt}}
\tikzset{eli/.style={ellipse, rotate=0, draw=black, fill=gray!20}}

%http://tex.stackexchange.com/questions/199683/how-to-plot-quantum-logical-gates-with-tikz
\tikzset{
cross/.style={path picture={ 
            \draw[thick,black](path picture bounding box.north) -- (path picture bounding                  box.south) (path picture bounding box.west) -- (path picture bounding                      box.east);
            }},
crossx/.style={path picture={ 
            \draw[thick,black,inner sep=0pt]
                (path picture bounding box.south east) -- (path picture bounding box.north west) (path picture bounding box.south west) -- (path picture bounding box.north east);
            }},
circlewc/.style={circle=2pt,draw, crossx}
}

==> commands/thms.tex <==
\newtheorem{LSM}{{\em Theorem: Lieb, Schultz, Mattis (1961)}}
\newtheorem{Oshikawa}{{\em Extension: Oshikawa (1999)}}
